A pullback diagram in the coarse category

This paper studies the asymptotic product of two metric spaces. It is well defined if one of the spaces is visual or if both spaces are geodesic. In this case the asymptotic product is the pullback of a limit diagram in the coarse category. Using this product construction we can define a homotopy theory on coarse metric spaces in a natural way. We prove that all finite colimits exist in the coarse category.

==> Homotopy.tex <==
\section{Homotopy}
\label{sec:homotopy}
\begin{defn}
Let $T$ be a metric space then 
 \[
 \digamma(T)=T\times \Z_+ 
 \]
 is a metric space with metric 
 \[
  d((x,i),(y,j))=\sqrt{i^2+j^2-(2-d_T(x,y)^2)ij}.
 \]
 Note that we impose that $\Z_+$ does not contain $0$ thus $d$ is a well defined 
metric. 
\end{defn}

\begin{rem}
 A countable subset $((x_i,n_i),(y_i,m_i))_i\s \digamma(T)^2$ is an entourage if
 \begin{enumerate}
  \item the set $(n_i,m_i)_i$ is an entourage in $\Z_+$
  \item and if $n_i\to \infty$ then there is some constant $c\ge 0$ such that $d(x_i,y_i)\le c/n_i$
 \end{enumerate}
 If $X$ is a metric space the asymptotic product $X\ast \digamma(T)$ is well defined provided the constant $R\ge 1$.
\end{rem}

\begin{defn}\name{coarse homotopy}
\label{defn:homotopy}
 Denote by $[0,1]$ the unit interval with the standard euclidean metric 
$d_{[0,1]}$. Let $X$ be a metric space and let $Y$ be a coarse space.
\begin{itemize}
\item Two coarse maps $f,g:X\to Y$ are said to be \emph{coarsely homotopic} if 
there is a coarse map $h:X\ast \digamma([0,1])\to Y$ such that $f$ is the 
restriction of $h$ to $X\ast \digamma(0)$ and $g$ is the restriction of $h$ to 
$X\ast \digamma(1)$.
\item A coarse map $f:X\to Y$ is a \emph{coarse homotopy equivalence} if there 
is a coarse map $g:Y\to X$ such that $f\circ g$ is coarsely homotopic to $id_Y$ 
and $g\circ f$ is coarsely homotopic to $id_X$.
\item Two coarse spaces $X,Y$ are called \emph{coarsely homotopy equivalent} if 
there is a coarse homotopy equivalence $f:X\to Y$.
\end{itemize}
\end{defn}

\begin{rem}
 There are other notions of homotopy in the coarse category but they differ from 
that one. 
\end{rem}

\begin{lem}
 If two coarse maps $f,g:X\to Y$ between metric spaces are close then they are 
coarsely homotopic.
\end{lem}
\begin{proof}
 We define a homotopy $h:X\ast \digamma([0,1])\to Y$ between $f$ and $g$ by
 \[
  h(x,(0,i))=f(x)
 \]
and for $1\ge t> 0$:
\[
 h(x,(t,i))=g(x).
\]
Now we just need to show that $h$ is a coarse map. First we show $h$ is coarsely uniform: if $t_i\to 0$ in $[0,1]$ such that $d(t_i,0)\le 
1/i$ and $(x_i)_i\s X$ a sequence of points then
 \[
  h((x_i,(t_i,i)),(x_i,(0,i))=\{(f(x_i),g(x_i)):i\}
 \]
 is an entourage.
The map $h$ is coarsely proper because $f,g$ are.
\end{proof}
% 
% \section{Acyclic Spaces}
% There is a notion of flasque spaces for which most coarse cohomology theories 
% vanish. Let us translate~\cite[Definition~3.6]{Willet2013} into coarse structure 
% notation:
% \begin{defn}
%  A coarse space $X$ is called \emph{flasque} if there is a coarse map $\phi:X\to 
% X$ such that
%  \begin{itemize}
%  \item $\phi$ is close to the identity on $X$;
%   \item for every bounded set $B\s X$ there is some $N_B\in \N$ such that 
%   \[
%    \phi^{\circ n}(X)\cap B=\emptyset
%   \]
%   for every $n\ge N_B$.
%   \item For every entourage $E$ the set $\bigcup_n\zzp{(\phi^{\circ n})}E$ is an 
% entourage.
%  \end{itemize}
% \end{defn}
% 
% \begin{thm}
% \label{thm:flasqueacyclic}
%  If $X$ is a flasque space then there is a coarse homotopy equivalence
%  \f{
%   \varPhi:X\times \Z_+&\to X\\
%   (x,i)&\mapsto \phi^{\circ i}(x).
%  }
%  Here $\phi^{\circ 0}$ denotes the identity on $X$.
% \end{thm}
% \begin{proof}
%  We show that the coarse homotopy inverse to $\varPhi$ is
% \f{
% i_0:X &\to X\times \Z_+\\
% x &\mapsto (x,0).
% }
% 
% Now $\varPhi\circ i_0=id_X$.
% 
% We show that $i_0\circ \varPhi$ and $id_{X\times \Z_+}$ are coarsely homotopic: 
% Define a map
% \f{
%  h:(X\times \Z_+)\ast \digamma([0,1])&\to X\times \Z_+\\
% ((x,i),(t,j))&\mapsto (\phi^{\circ\lfloor ti\rfloor}(x),\lfloor(1-t)i\rfloor).
%  }
%  We show that $h$ is a coarse map:
%  \begin{enumerate}
%  \item $h$ is coarsely uniform: let $E\s ((X\times \Z_+)\ast \digamma([0,1]))^2$ 
% be an entourage. Denote by $p_X:X\times \Z_+\to X$ and $p_{\Z_+}:X\times\Z_+\to 
% \Z_+$ the projections to $X,\Z_+$, both $p_X,p_{\Z_+}$ are coarsely uniform 
% maps. We show $\zz{p_X}\circ\zz h(E)$ is an entourage and $\zz p_{\Z_+}\circ \zz 
% h(E)$ is an entourage. Note:
%  \[
%   \zz {p_X}\circ \zz h(E)\s \bigcup_n(\phi^{\circ n})^2(E)
%  \]
% is an entourage. If $i,j\in \Z_+,t,s\in [0,1]$ then
% \f{
% |\lfloor (1-t)i\rfloor-\lfloor (1-s)j\rfloor|
% &\le |(1-t)i-(1-s)j|+2\\
% &\le |i-j|+2
% }
% Thus $\zz{p_{\Z_+}}\circ \zz h(E)$ is an entourage.
%  \item $h$ is coarsely proper: Let $B\s X\times \Z_+$ be a bounded subset. We 
% write
%  \[
%   B=\bigcup_i B_i\times i
%  \]
%  which is a finite union. Then for every $i$ there is some $N_i$ such that
%  \[
%  \phi^{\circ n}(X)\cap B_i=\emptyset
%  \]
% for every $n\ge N_i$. We show $p_X\circ h^{-1}(B)$ and $p_{\Z_+}\circ h^{-1}(B)$ 
% is bounded Then
% \[
% \iip h B\s (p_X\circ \iip h B\times p_{\Z_+}\circ \iip h B)\ast \digamma([0,1])
% \]
% is bounded in $(X\times\Z_+)\ast \digamma([0,1])$. Now
% \[
% p_X\circ \iip h B\s \bigcup_i (\phi^{\circ-0}(B_i)\cup\cdots\cup\phi^{\circ- 
% N_i}(B_i))
% \]
% is bounded in $X$. If $j\in p_{\Z_+}\circ \iip h B$ then $\lfloor tj\rfloor \le 
% N_i$ for at least one $i$. Thus
% \[
%  j\le \max_i N_i
% \]
% therefore $p_{\Z_+}\circ \iip h B$ is bounded in $\Z_+$.
%  \end{enumerate}
% \end{proof}
% 
% \begin{ex}
%  Note that $\Z_+$ is flasque by
%  \f{
%  \phi:\Z_+&\to \Z_+\\
%   n&\mapsto n+1.
%  }
%  Thus there is a coarse homotopy equivalence $\Z_+^2\to \Z_+$. Now for every $n$ 
% the space $\Z_+^n$ is flasque. As a result $\Z_+^n$ is coarsely homotopy 
% equivalent to $\Z_+$ for every $n$.
% \end{ex}

